The Carnegie-Irvine Galaxy Survey. IX. Classification of Bulge Types and Statistical Properties of Pseudo Bulges

We study the statistical properties of 320 bulges of disk galaxies in the Carnegie-Irvine Galaxy Survey, using robust structural parameters of galaxies derived from image fitting. We apply the Kormendy relation to classify classical and pseudo bulges and characterize bulge dichotomy with respect to bulge structural properties and physical properties of host galaxies. We confirm previous findings that pseudo bulges on average have smaller S\'{e}rsic indices, smaller bulge-to-total ratios, and fainter surface brightnesses when compared with classical bulges. Our sizable sample statistically shows that pseudo bulges are more intrinsically flattened than classical bulges. Pseudo bulges are most frequent (incidence $\gtrsim 80\%$) in late-type spirals (later than Sc). Our measurements support the picture in which pseudo bulges arose from star formation induced by inflowing gas, while classical bulges were born out of violent processes such as mergers and coalescence of clumps. We reveal differences with the literature that warrant attention: (1) the bimodal distribution of S\'{e}rsic indices presented by previous studies is not reproduced in our study; (2) classical and pseudo bulges have similar relative bulge sizes; and (3) the pseudo bulge fraction is considerably smaller in early-type disks compared with previous studies based on one-dimensional surface brightness profile fitting. We attribute the above differences to our improved image quality, more robust bulge-to-disk decomposition technique, and different classification criteria applied. Moreover, we find that barred galaxies do not host more pseudo bulges or more prominent pseudo bulges than unbarred galaxies. Various implications of these findings are discussed.

==> mrt_temp.tex <==
ESO 185-G054 & $20.94\pm 0.20$ & $4.94\pm 0.26$ & $ 65.03\pm  8.54$ & $0.269\pm 0.000$ \\
IC 1459      & $19.36\pm 0.09$ & $5.19\pm 0.12$ & $ 50.68\pm  2.58$ & $0.261\pm 0.000$ \\
IC 1633      & $21.60\pm 0.25$ & $6.69\pm 0.34$ & $ 75.45\pm 11.86$ & $0.167\pm 0.000$ \\
IC 2311      & $19.53\pm 0.19$ & $5.18\pm 0.29$ & $ 22.86\pm  2.68$ & $0.043\pm 0.000$ \\
IC 2597      & $20.53\pm 0.12$ & $4.97\pm 0.17$ & $ 40.53\pm  3.09$ & $0.284\pm 0.000$ \\
IC 3370      & $19.79\pm 0.08$ & $3.92\pm 0.15$ & $ 33.33\pm  1.72$ & $0.164\pm 0.000$ \\
IC 3896      & $20.57\pm 0.29$ & $5.49\pm 0.42$ & $ 50.52\pm  9.39$ & $0.208\pm 0.002$ \\
IC 4296      & $20.44\pm 0.19$ & $4.97\pm 0.23$ & $ 55.59\pm  6.47$ & $0.084\pm 0.001$ \\
IC 4742      & $20.31\pm 0.29$ & $3.89\pm 0.51$ & $ 29.29\pm  6.04$ & $0.192\pm 0.002$ \\
IC 4765      & $22.77\pm 0.59$ & $6.05\pm 0.66$ & $183.98\pm 76.13$ & $0.362\pm 0.001$ \\
IC 4797      & $18.93\pm 0.09$ & $4.52\pm 0.16$ & $ 22.95\pm  1.34$ & $0.399\pm 0.001$ \\
IC 4889      & $19.16\pm 0.06$ & $4.07\pm 0.09$ & $ 26.47\pm  0.95$ & $0.336\pm 0.000$ \\
IC 5328      & $19.66\pm 0.12$ & $4.26\pm 0.19$ & $ 29.39\pm  2.17$ & $0.288\pm 0.002$ \\
NGC 596      & $19.71\pm 0.06$ & $5.14\pm 0.10$ & $ 33.05\pm  1.21$ & $0.126\pm 0.001$ \\
NGC 636      & $20.29\pm 0.23$ & $6.42\pm 0.40$ & $ 37.62\pm  5.12$ & $0.119\pm 0.000$ \\
NGC 720      & $18.90\pm 0.07$ & $3.22\pm 0.09$ & $ 37.62\pm  1.73$ & $0.420\pm 0.000$ \\
NGC 1052     & $18.95\pm 0.06$ & $3.97\pm 0.10$ & $ 31.21\pm  1.09$ & $0.295\pm 0.000$ \\
NGC 1172     & $21.22\pm 0.86$ & $ NaN\pm  NaN$ & $ 59.63\pm 28.91$ & $0.207\pm 0.002$ \\
NGC 1199     & $19.92\pm 0.13$ & $4.61\pm 0.20$ & $ 31.27\pm  2.38$ & $0.249\pm 0.001$ \\
NGC 1209     & $19.03\pm 0.05$ & $4.58\pm 0.10$ & $ 24.90\pm  0.82$ & $0.524\pm 0.000$ \\
NGC 1339     & $18.91\pm 0.08$ & $4.58\pm 0.16$ & $ 17.61\pm  0.85$ & $0.284\pm 0.000$ \\
NGC 1340     & $19.18\pm 0.07$ & $3.59\pm 0.12$ & $ 39.78\pm  1.91$ & $0.354\pm 0.000$ \\
NGC 1374     & $19.51\pm 0.05$ & $4.62\pm 0.09$ & $ 28.28\pm  0.94$ & $0.097\pm 0.000$ \\
NGC 1379     & $19.61\pm 0.05$ & $3.12\pm 0.08$ & $ 28.17\pm  0.87$ & $0.019\pm 0.000$ \\
NGC 1395     & $19.72\pm 0.09$ & $4.33\pm 0.12$ & $ 55.52\pm  3.15$ & $0.163\pm 0.001$ \\
NGC 1399     & $19.68\pm 0.10$ & $4.58\pm 0.12$ & $ 64.74\pm  3.87$ & $0.093\pm 0.001$ \\
NGC 1404     & $18.10\pm 0.11$ & $3.31\pm 0.18$ & $ 23.72\pm  1.64$ & $0.136\pm 0.001$ \\
NGC 1407     & $20.35\pm 0.14$ & $4.42\pm 0.17$ & $ 80.68\pm  7.34$ & $0.046\pm 0.000$ \\
NGC 1426     & $19.91\pm 0.18$ & $5.09\pm 0.33$ & $ 34.23\pm  3.82$ & $0.350\pm 0.000$ \\
NGC 1427     & $20.15\pm 0.11$ & $5.45\pm 0.18$ & $ 47.76\pm  3.48$ & $0.299\pm 0.000$ \\
NGC 1439     & $21.09\pm 0.41$ & $ NaN\pm  NaN$ & $ 58.96\pm 13.42$ & $0.090\pm 0.000$ \\
NGC 1453     & $20.36\pm 0.20$ & $5.63\pm 0.29$ & $ 43.13\pm  5.39$ & $0.163\pm 0.001$ \\
NGC 1521     & $20.42\pm 0.18$ & $5.25\pm 0.26$ & $ 39.67\pm  4.45$ & $0.300\pm 0.001$ \\
NGC 1549     & $19.67\pm 0.10$ & $4.96\pm 0.14$ & $ 58.35\pm  3.67$ & $0.103\pm 0.000$ \\
NGC 1600     & $20.44\pm 0.20$ & $3.75\pm 0.27$ & $ 51.52\pm  7.17$ & $0.329\pm 0.002$ \\
NGC 1700     & $19.24\pm 0.17$ & $5.33\pm 0.28$ & $ 27.45\pm  2.85$ & $0.287\pm 0.000$ \\
NGC 2305     & $19.90\pm 0.14$ & $4.82\pm 0.19$ & $ 29.08\pm  2.52$ & $0.251\pm 0.000$ \\
NGC 2325     & $20.50\pm 0.11$ & $2.95\pm 0.12$ & $ 50.43\pm  3.71$ & $0.364\pm 0.000$ \\
NGC 2434     & $20.40\pm 0.18$ & $4.71\pm 0.27$ & $ 39.65\pm  4.53$ & $0.089\pm 0.001$ \\
NGC 2663     & $21.03\pm 0.29$ & $4.73\pm 0.35$ & $ 99.12\pm 19.30$ & $0.332\pm 0.001$ \\
NGC 2865     & $18.66\pm 0.17$ & $ NaN\pm  NaN$ & $ 15.06\pm  1.79$ & $0.250\pm 0.000$ \\
NGC 2986     & $20.60\pm 0.11$ & $5.57\pm 0.17$ & $ 62.50\pm  4.44$ & $0.151\pm 0.000$ \\
NGC 3078     & $19.43\pm 0.17$ & $5.00\pm 0.27$ & $ 29.47\pm  3.05$ & $0.241\pm 0.000$ \\
NGC 3087     & $19.93\pm 0.16$ & $5.33\pm 0.24$ & $ 32.10\pm  3.16$ & $0.149\pm 0.000$ \\
NGC 3091     & $20.34\pm 0.19$ & $5.24\pm 0.27$ & $ 46.07\pm  5.62$ & $0.286\pm 0.001$ \\
NGC 3136     & $21.32\pm 0.43$ & $6.73\pm 0.58$ & $107.32\pm 30.36$ & $0.264\pm 0.001$ \\
NGC 3250     & $19.53\pm 0.12$ & $3.85\pm 0.17$ & $ 32.48\pm  2.40$ & $0.256\pm 0.001$ \\
NGC 3258     & $20.39\pm 0.20$ & $4.80\pm 0.26$ & $ 39.05\pm  4.89$ & $0.127\pm 0.001$ \\
NGC 3268     & $21.48\pm 0.50$ & $5.51\pm 0.61$ & $ 73.56\pm 25.03$ & $0.203\pm 0.000$ \\
NGC 3557     & $19.80\pm 0.10$ & $4.58\pm 0.13$ & $ 46.45\pm  2.78$ & $0.242\pm 0.000$ \\
NGC 3585     & $20.15\pm 0.17$ & $6.24\pm 0.25$ & $ 96.35\pm 10.06$ & $0.445\pm 0.001$ \\
NGC 3923     & $20.43\pm 0.14$ & $4.71\pm 0.17$ & $105.46\pm  9.57$ & $0.343\pm 0.001$ \\
NGC 3962     & $20.09\pm 0.11$ & $4.91\pm 0.16$ & $ 50.80\pm  3.69$ & $0.202\pm 0.000$ \\
NGC 4696     & $21.02\pm 0.12$ & $2.99\pm 0.13$ & $ 91.29\pm  8.00$ & $0.219\pm 0.000$ \\
NGC 4709     & $21.64\pm 0.38$ & $5.70\pm 0.47$ & $ 86.14\pm 21.23$ & $0.155\pm 0.000$ \\
NGC 4742     & $18.17\pm 0.08$ & $7.99\pm 0.17$ & $ 17.35\pm  0.79$ & $0.400\pm 0.000$ \\
NGC 4760     & $20.84\pm 0.19$ & $4.42\pm 0.25$ & $ 47.78\pm  6.06$ & $0.155\pm 0.001$ \\
NGC 4767     & $19.51\pm 0.10$ & $4.17\pm 0.16$ & $ 28.67\pm  1.87$ & $0.423\pm 0.001$ \\
NGC 4786     & $19.46\pm 0.10$ & $4.08\pm 0.16$ & $ 22.61\pm  1.44$ & $0.232\pm 0.000$ \\
NGC 4936     & $20.42\pm 0.17$ & $4.14\pm 0.22$ & $ 53.87\pm  6.20$ & $0.170\pm 0.001$ \\
NGC 4976     & $19.50\pm 0.37$ & $ NaN\pm  NaN$ & $ 53.50\pm 13.47$ & $0.320\pm 0.001$ \\
NGC 5011     & $20.42\pm 0.15$ & $5.06\pm 0.22$ & $ 36.71\pm  3.48$ & $0.158\pm 0.000$ \\
NGC 5018     & $18.77\pm 0.06$ & $4.39\pm 0.10$ & $ 24.54\pm  0.90$ & $0.297\pm 0.000$ \\
NGC 5044     & $20.45\pm 0.12$ & $3.12\pm 0.14$ & $ 50.18\pm  4.20$ & $0.060\pm 0.000$ \\
NGC 5061     & $19.67\pm 0.15$ & $6.48\pm 0.25$ & $ 45.16\pm  4.18$ & $0.099\pm 0.001$ \\
NGC 5077     & $19.27\pm 0.14$ & $4.56\pm 0.21$ & $ 29.59\pm  2.56$ & $0.302\pm 0.001$ \\
NGC 5328     & $19.96\pm 0.14$ & $5.23\pm 0.21$ & $ 31.56\pm  2.63$ & $0.313\pm 0.000$ \\
NGC 5419     & $20.82\pm 0.18$ & $4.55\pm 0.23$ & $ 69.53\pm  8.57$ & $0.210\pm 0.000$ \\
NGC 5791     & $19.44\pm 0.09$ & $3.98\pm 0.15$ & $ 25.11\pm  1.46$ & $0.425\pm 0.000$ \\
NGC 5796     & $19.82\pm 0.14$ & $5.06\pm 0.22$ & $ 28.20\pm  2.45$ & $0.131\pm 0.000$ \\
NGC 5812     & $19.55\pm 0.10$ & $5.24\pm 0.17$ & $ 26.99\pm  1.70$ & $0.044\pm 0.000$ \\
NGC 5898     & $19.66\pm 0.20$ & $4.59\pm 0.28$ & $ 27.05\pm  3.39$ & $0.019\pm 0.001$ \\
NGC 5903     & $20.86\pm 0.24$ & $4.87\pm 0.31$ & $ 58.88\pm  9.02$ & $0.232\pm 0.000$ \\
NGC 6851     & $19.00\pm 0.07$ & $4.20\pm 0.14$ & $ 16.99\pm  0.78$ & $0.266\pm 0.000$ \\
NGC 6868     & $20.20\pm 0.18$ & $4.94\pm 0.23$ & $ 54.46\pm  6.05$ & $0.186\pm 0.000$ \\
NGC 6876     & $20.32\pm 0.08$ & $3.05\pm 0.10$ & $ 46.76\pm  2.67$ & $0.136\pm 0.000$ \\
NGC 6909     & $20.14\pm 0.14$ & $4.37\pm 0.25$ & $ 32.45\pm  2.97$ & $0.442\pm 0.000$ \\
NGC 6958     & $19.29\pm 0.07$ & $5.17\pm 0.11$ & $ 22.14\pm  0.97$ & $0.144\pm 0.000$ \\
NGC 7029     & $19.51\pm 0.07$ & $5.23\pm 0.11$ & $ 27.04\pm  1.08$ & $0.364\pm 0.000$ \\
NGC 7145     & $20.49\pm 0.15$ & $4.94\pm 0.21$ & $ 39.35\pm  3.78$ & $0.036\pm 0.000$ \\
NGC 7196     & $19.34\pm 0.13$ & $4.58\pm 0.21$ & $ 24.41\pm  1.89$ & $0.217\pm 0.000$ \\
NGC 7507     & $18.93\pm 0.09$ & $4.99\pm 0.13$ & $ 37.67\pm  1.98$ & $0.038\pm 0.000$ \\
NGC 7796     & $20.05\pm 0.13$ & $4.91\pm 0.19$ & $ 33.59\pm  2.72$ & $0.153\pm 0.000$ \\

